Effects of Turbulence Induced Scattering on Underwater Optical Wireless Communications

This paper presents a comprehensive description of the relative effect of optical underwater turbulence in combination with absorption and scattering. Turbulence induced scattering is shown to cause and increase both spatial and temporal spreading at the receiver plane. It is also demonstrated that the relative impact of turbulence on a received signal is lower in a highly scattering channel. Received intensity distributions are presented confirming that fluctuations in received power from this method follow the commonly used Log-Normal fading model. The impact of turbulence induced scattering on maximum achievable data rate in the underwater channel is investigated.

==> subfigure_script_dump.tex <==
\begin{figure*}[p!]
\centering
\begin{subfigure}[h]{0.45\textwidth}
	\includegraphics[width=\textwidth]{dgf_fit_coast30bt0}
	\caption{$b_t=0$~m\textsuperscript{-1}}
	\label{0coast30}
\end{subfigure}
~
\begin{subfigure}[h]{0.45\textwidth}
	\includegraphics[width=\textwidth]{dgf_fit_coast30bt005}
	\caption{$b_t=0.5$~m\textsuperscript{-1}}
	\label{05coast30}
\end{subfigure}
\\
\begin{subfigure}[h]{0.45\textwidth}
	\includegraphics[width=\textwidth]{dgf_fit_coast30bt01}
	\caption{$b_t=1$~m\textsuperscript{-1}}
	\label{1coast30}
\end{subfigure}
~
\begin{subfigure}[h]{0.45\textwidth}
	\includegraphics[width=\textwidth]{dgf_fit_coast30bt02}
	\caption{$b_t=2$~m\textsuperscript{-1}}
	\label{2coast30}
\end{subfigure}
\caption{Double-Gamma function fitted impulse responses for a 30~m link in coastal water.}
\label{coastir}
\end{figure*}

\begin{figure*}[p!]
	\centering
	\begin{subfigure}[h]{0.45\textwidth}
		\includegraphics[width=\textwidth]{dgf_fit_harbour15bt0}
		\caption{$b_t=0$~m\textsuperscript{-1}}
		\label{0harbour15}
	\end{subfigure}
	~
	\begin{subfigure}[h]{0.45\textwidth}
		\includegraphics[width=\textwidth]{dgf_fit_harbour15bt05}
		\caption{$b_t=0.5$~m\textsuperscript{-1}}
		\label{05harbour15}
	\end{subfigure}
	\\
	\begin{subfigure}[h]{0.45\textwidth}
		\includegraphics[width=\textwidth]{dgf_fit_harbour15bt1}
		\caption{$b_t=1$~m\textsuperscript{-1}}
		\label{1harbour15}
	\end{subfigure}
	~
	\begin{subfigure}[h]{0.45\textwidth}
		\includegraphics[width=\textwidth]{dgf_fit_harbour15bt2}
		\caption{$b_t=2$~m\textsuperscript{-1}}
		\label{2harbour15}
	\end{subfigure}
	\caption{Double-Gamma function fitted impulse responses for a 15~m link in harbour water.}
	\label{harbourir}
\end{figure*}
